Improved Sample Complexity Analysis For First Order Bilevel Reinforcement Learning

Bilevel reinforcement learning optimizes an upper-level objective through the policy response to a lower-level reinforcement learning problem. Such problems arise when learning a reward model while adapting a policy to that reward. However, a gap remains between sample-complexity guarantees and practical actor--critic training. Tabular analyses restrict applicability to finite spaces, while continuous-state analyses often impose a uniform Polyak--\L{}ojasiewicz (PL) condition. We show that this condition need not hold even for smooth positive policies with exactly representable values. We develop a single-loop, fully first-order method for continuous states and finite actions with specified multilayer neural actors and a persistently trained nonlinear critic built from fixed features. Under explicit initialization, regularity, feature-excitation, and value-realizability conditions, fixed reference-KL regularization yields local curvature, and we prove containment of the coupled iterates. Shared trajectories control sampling noise, while paired critic analysis controls normalized critic-error differences as the response perturbation shrinks. A joint descent and tracking argument establishes an improved $\widetilde{\mathcal O}(\varepsilon^{-2})$ sample complexity for $O(\varepsilon)$ expected squared gradient norm of the upper objective induced by the selected regularized policy response, including critic training.

==> Makefile <==
.PHONY: all check clean

all: main.pdf

main.pdf: main.tex macros.tex references.bib iclr2027_conference.sty iclr2027_conference.bst $(wildcard sections/*.tex) $(wildcard appendix/*.tex) $(wildcard figures/*.pdf) $(wildcard tables/*.tex)
	latexmk -pdf -interaction=nonstopmode -halt-on-error main.tex

check: main.pdf
	python3 -c "from pathlib import Path; import re; s=Path('main.log').read_text(); m=re.search(r'ICLR-MAIN-TEXT-PAGES=(\d+)',s); assert m and int(m[1])<=9, 'Main text exceeds nine pages'; assert not re.search(r'undefined|multiply defined|Overfull',s), 'Resolve compilation diagnostics'; print('Build checks passed; main pages:',m[1])"

clean:
	latexmk -C


==> empirical_assets/continuous/paper_tables/scaling.tex <==
\begin{tabular}{rrrr}
\toprule
$T$ & $N$ (millions) & Zero: $\overline G_T$ & Displaced: $\overline G_T$ \\
\midrule
2000 & 4.100 & $9.440\pm0.206$ & $9.182\pm0.231$ \\
4000 & 8.197 & $6.650\pm0.127$ & $6.455\pm0.123$ \\
8000 & 16.388 & $4.687\pm0.074$ & $4.553\pm0.067$ \\
16000 & 32.771 & $3.305\pm0.050$ & $3.211\pm0.041$ \\
\bottomrule
\end{tabular}


==> empirical_assets/continuous/paper_tables/training.tex <==
\begin{tabular}{lrrr}
\toprule
Variant & Final $x$ & Final $G$ ($10^{-6}$) & $\overline G_T$ ($10^{-4}$) \\
\midrule
Full: zero & $0.539883\pm0.006173$ & $1.729\pm1.510$ & $9.403\pm0.111$ \\
Full: displaced & $0.539954\pm0.006203$ & $1.737\pm1.507$ & $9.190\pm0.139$ \\
No chain & $0.548919\pm0.006659$ & $3.069\pm3.085$ & $9.327\pm0.132$ \\
Exact value & $0.540346\pm0.006304$ & $1.769\pm1.353$ & $9.403\pm0.127$ \\
\bottomrule
\end{tabular}


==> empirical_assets/continuous/paper_tables/tuples.tex <==
\begin{tabular}{rrrr}
\toprule
ID & $x$ & $\Delta U$ & $S$ \\
\midrule
0 & $0.2$ & $(0,0)$ & $(0.15,-0.2)$ \\
1 & $0.4$ & $(0.08,-0.03)$ & $(-0.2,0.1)$ \\
2 & $0.55$ & $(-0.06,0.08)$ & $(0.1,0.2)$ \\
3 & $0.7$ & $(0.02,0.04)$ & $(-0.15,-0.1)$ \\
4 & $-0.35$ & $(0.05,0.02)$ & $(0.25,-0.15)$ \\
5 & $0.9$ & $(-0.04,-0.04)$ & $(-0.1,0.3)$ \\
\bottomrule
\end{tabular}


==> macros.tex <==
\usepackage[T1]{fontenc}
\usepackage{times}
\usepackage{microtype}
\usepackage{amsmath,amssymb,amsthm,mathtools,bm,mathrsfs}
\usepackage{aliascnt}
\usepackage{booktabs,array,tabularx,multirow,longtable}
\usepackage{enumitem}
\usepackage{graphicx}
\usepackage{placeins}
\usepackage{xcolor}
\usepackage{url}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{hyperref}
\usepackage{subcaption}
\bibliographystyle{iclr2027_conference}
\usepackage[nameinlink,noabbrev,capitalise]{cleveref}
\hypersetup{colorlinks=true,linkcolor=blue!45!black,citecolor=blue!45!black,urlcolor=blue!45!black}
\newtheorem{theorem}{Theorem}[section]
\newaliascnt{proposition}{theorem}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\newaliascnt{corollary}{theorem}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\newaliascnt{assumption}{theorem}
\newtheorem{assumption}[assumption]{Assumption}
\aliascntresetthe{assumption}
\newaliascnt{condition}{theorem}
\newtheorem{condition}[condition]{Condition}
\aliascntresetthe{condition}
\theoremstyle{definition}
\newaliascnt{definition}{theorem}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}
\theoremstyle{remark}
\newaliascnt{remark}{theorem}
\newtheorem{remark}[remark]{Remark}
\aliascntresetthe{remark}
\crefname{theorem}{Theorem}{Theorems}
\Crefname{theorem}{Theorem}{Theorems}
\crefname{proposition}{Proposition}{Propositions}
\Crefname{proposition}{Proposition}{Propositions}
\crefname{lemma}{Lemma}{Lemmas}
\Crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\Crefname{corollary}{Corollary}{Corollaries}
\crefname{assumption}{Assumption}{Assumptions}
\Crefname{assumption}{Assumption}{Assumptions}
\crefname{condition}{Condition}{Conditions}
\Crefname{condition}{Condition}{Conditions}
\crefname{definition}{Definition}{Definitions}
\Crefname{definition}{Definition}{Definitions}
\crefname{remark}{Remark}{Remarks}
\Crefname{remark}{Remark}{Remarks}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\op}{\mathrm{op}}
\newcommand{\Cov}{\operatorname{Cov}}
\newcommand{\Var}{\operatorname{Var}}
\newcommand{\argmin}{\operatorname*{arg\,min}}
\newcommand{\grad}{\nabla}
\newcommand{\wtO}{\widetilde{\mathcal O}}
\newcommand{\ip}[2]{\left\langle #1,#2\right\rangle}
\newcommand{\norm}[1]{\left\lVert #1\right\rVert}
\newcommand{\abs}[1]{\left\lvert #1\right\rvert}
\newcommand{\given}{\,\middle|\,}
\newcommand{\Id}{I}
\newcommand{\piRef}{\pi_{\mathrm{ref}}}
\newcommand{\eps}{\varepsilon}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Fisher}{\mathcal F}
\newcommand{\dbar}{\overline d}
\newcommand{\mmin}{m_{\min}}
\newcommand{\ddeep}{\delta_{\mathbf m,L}}
\newcommand{\calL}{\mathcal L}
\newcommand{\epspair}{\varepsilon_{\mathrm{pair}}}
\newcommand{\epsprox}{\varepsilon_{\mathrm{prox}}}
\newcommand{\epscrit}{\varepsilon_{\mathrm{crit}}}
\newcommand{\epsH}{\varepsilon_H}
\newcommand{\epsV}{\varepsilon_V}
\newcommand{\epsTr}{\varepsilon_{\mathrm{tr}}}
\newcommand{\method}{\textsc{Chain-Pair}}
\newcommand{\todoresult}[1]{\fbox{\parbox{.94\linewidth}{\small\textbf{Empirical placeholder.} #1}}}
\setlist[itemize]{leftmargin=1.35em,itemsep=.15em,topsep=.25em}
\setlist[enumerate]{leftmargin=1.55em,itemsep=.15em,topsep=.25em}
\newcommand{\Pp}{\mathbb{P}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\ThetaR}{\Theta_R}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\Bgeom}{\mathcal B_{\mathrm{geom}}}
\newcommand{\Dstab}{\mathcal D_{\mathrm{stab}}}
\newcommand{\dist}{\operatorname{dist}}
\newcommand{\tauExit}{\tau_{\mathrm{exit}}}
\newcommand{\PhiStar}{\Phi_\star}
\newcommand{\Floor}{\mathsf{Floor}}
\newcommand{\FloorLoc}{\mathsf{Floor}_{\mathrm{loc}}}
\newcommand{\cD}{\mathcal D}
\usepackage{pifont}
\newcommand{\xmark}{\ding{55}}
\newcommand{\Prb}{\mathbb{P}}

\crefname{algorithm}{Algorithm}{Algorithms}
\Crefname{algorithm}{Algorithm}{Algorithms}
\newcommand{\CriticAppendix}{Appendix~\ref{app:main-results}}
\newcommand{\piref}{\pi_{\mathrm{ref}}}
\newcommand{\AQ}{\mathcal A_Q}
\newcommand{\CritSet}{\mathcal K_Q}
\newcommand{\Prob}{\mathbb P}
\newcommand{\sym}{\operatorname{sym}}
\newcommand{\poly}{\operatorname{poly}}
\newcommand{\CT}{\mathcal C}
\newcommand{\AT}{\mathcal T}
\newcommand{\LT}{\mathcal D}
\newcommand{\Hist}{\mathcal F}


==> sections/03_problem_formulation_updated.tex <==
\section{Problem Formulation}
\label{sec:main-setup}

\paragraph{Problem Setup}
For an upper parameter $x\in\cO_x=\R^{d_x}$, let $\mathcal M_x=(\cS,\cA,P,r_x,\rho,\gamma)$ be a discounted Markov decision process: $\cS$ is the compact, possibly continuous state space; $\cA$ the finite action set; $P(ds'\mid s,a)$ the transition law; $r_x(s,a)$ the reward; $\rho$ the initial-state law; and $\gamma\in(0,1)$ the discount. Only the reward and upper loss depend on $x$.

\paragraph{Multilayer neural actor.}
Let $L$ be the actor's hidden depth, $\mathbf m=(m_1,\ldots,m_L)$ its hidden widths, and $\alpha\in\R^r$ its trainable coordinates. A scalar neural score $F_{\mathbf m,\alpha}(s,a)$ modifies a fixed strictly positive reference policy $\piRef$ to define the action probabilities
\begin{equation}
 \pi_{\mathbf m,\alpha}(a\mid s)
 =\frac{\piRef(a\mid s)e^{F_{\mathbf m,\alpha}(s,a)}}
 {\sum_{b\in\cA}\piRef(b\mid s)e^{F_{\mathbf m,\alpha}(s,b)}}.
 \label{eq:main-policy}
\end{equation}
The score uses two coupled smooth multilayer networks whose weights vary through the same $r$ coordinates around initialization. Depth $L$ and dimension $r$ stay fixed as widths vary.$F_{\mathbf m,0}=0$ gives $\pi_{\mathbf m,0}=\piRef$. Appendix~\ref{app:actor-construction} specifies the coupling, normalization, inputs, and activation requirements.

\paragraph{Why the actor restriction matters.}\label{ex:main-PL}
Prior works such as \citet{gaur2025sample} require a lower-level PL condition that requires small policy gradients to imply
small optimality gaps. The example below shows that smoothness,
positive action probabilities, and exact value representation alone
do not ensure this property: the policy parameterization can introduce
suboptimal stationary points.
Consider a one-state self-loop MDP with rewards $r(1)=1$, $r(0)=0$, set $\pi_\theta(1)=\tfrac12+\tfrac14\sin\theta$ and $\pi_\theta(0)=1-\pi_\theta(1)$ for $\theta\in[-\pi,\pi]$. The normalized return is $J(\theta)=\pi_\theta(1)$; define $J^*=\max_{\theta\in[-\pi,\pi]}J(\theta)$. A uniform maximization Polyak-\L{}ojasiewicz (PL) condition bounds $J^*-J(\theta)$ by a fixed positive multiple of $|J'(\theta)|^2$. Yet $J'(-\pi/2)=0$ and $J^*-J(-\pi/2)=1/2$, despite smooth positive policies and exact value representation (\cref{prop:PL-counterexample}). Appendix~\ref{app:pl-strengthened} gives an additional example with a spurious strict local minimum for every positive reference-KL coefficient, together with a vanishing-Jacobian obstruction for multilayer neural policies.  This motivates our explicit actor
architecture and initialization, for which we derive local response
curvature under the stated assumptions and prove that the iterates
remain in the region where it holds.

\paragraph{Trajectories, feedback, and objectives.}
Let $\mathbb P_{\mathbf m,\alpha}$ be the law generated by $s_0\sim\rho$, $a_t\sim\pi_{\mathbf m,\alpha}(\cdot\mid s_t)$, and $s_{t+1}\sim P(\cdot\mid s_t,a_t)$; $\E_{\mathbf m,\alpha}$ denotes its expectation. Fix positive integers $I,K$ independently of accuracy. Let $\mathbb P^K_{\mathbf m,\alpha}$ be the law of the first $K$ actions and their states. A tuple $\boldsymbol\xi=(\xi^1,\ldots,\xi^I)$ contains $I$ independent such trajectories; $\otimes I$ denotes their product law. Feedback $Y$ follows a fixed conditional law $\mathcal D(\cdot\mid\boldsymbol\xi)$, independent of $(x,\alpha)$ given the tuple. Let $L(x;\boldsymbol\xi,Y)$ be a sample loss. For fixed $\tau>0$, define the lower cost with reference Kullback--Leibler (KL) regularization and the upper loss by
\begin{align}
 g_{\tau,\mathbf m}(x,\alpha)
 &=(1-\gamma)\E_{\mathbf m,\alpha}\sum_{t\ge0}\gamma^t
 \left[-r_x(s_t,a_t)+\tau\log
 \frac{\pi_{\mathbf m,\alpha}(a_t\mid s_t)}{\piRef(a_t\mid s_t)}\right],
 \label{eq:main-lower}\\
 f_{\mathbf m}(x,\alpha)
 &=\E_{\boldsymbol\xi\sim(\mathbb P^K_{\mathbf m,\alpha})^{\otimes I},\,
 Y\sim\mathcal D(\cdot\mid\boldsymbol\xi)}L(x;\boldsymbol\xi,Y).
 \label{eq:main-upper}
\end{align}
The trajectory distribution makes $f_{\mathbf m}$ policy dependent.

For Bradley--Terry comparisons, $I=2$ and $Y\in\{0,1\}$, with $Y=1$ indicating preference for $\xi^1$. Writing $(s_t^i,a_t^i)$ for trajectory $i$, define the reward contrast and negative log-likelihood loss by
\begin{equation}
 \Delta_x=\sum_{t=0}^{K-1}\bigl[r_x(s_t^1,a_t^1)-r_x(s_t^2,a_t^2)\bigr],\qquad
 L(x;\boldsymbol\xi,Y)=\log(1+e^{\Delta_x})-Y\Delta_x.
 \label{eq:main-BT}
\end{equation}
Appendix~\ref{app:support-preference} verifies the loss bounds; no correctness of the fitted preference model is assumed.

\paragraph{Selected response and optimization target.}
Write $\nabla_x,\nabla_\alpha$ for partial gradients and $\Bgeom=\{\alpha\in\R^r:\|\alpha\|_2<R_{\rm geom}\}$ for a neighborhood of radius $R_{\rm geom}>0$. Under Section~\ref{sec:main-result}'s conditions, a suitable radius and fixed $\tau$ give a unique smooth local response $\alpha_{0,\mathbf m}^*(x)\in\Bgeom$ and upper objective $\Phi_{\tau,\mathbf m}$ satisfying
\begin{equation}
 \nabla_\alpha g_{\tau,\mathbf m}(x,\alpha_{0,\mathbf m}^*(x))=0,
 \qquad \Phi_{\tau,\mathbf m}(x)=f_{\mathbf m}(x,\alpha_{0,\mathbf m}^*(x)).
 \label{eq:main-local-response-root}
\end{equation}
We seek stationarity for $\min_{x\in\R^{d_x}}\Phi_{\tau,\mathbf m}(x)$. Subscript $0$ denotes the unperturbed response. The ball certifies a local minimizer; the actor domain remains $\R^r$. 

% The preference objective is an on-policy prediction risk. 

% Policy-dependent comparison entropy can shift its stationary point away from a correctly specified teacher reward; reward recovery and teacher-return optimality are separate objectives (\cref{crex:rem:preference-risk}).

\paragraph{Neural critic.}
The critic approximates the expected discounted sum of the per-step cost in \eqref{eq:main-lower}, conditional on an initial state--action pair and without the prefactor $1-\gamma$. Given a fixed bounded feature map $\varphi_Q:\cS\times\cA\to\R^{d_Q}$, trainable coordinates $\theta\in\R^{d_Q}$, and scale $m_Q\ge1$, use
\begin{equation}
 Q_{m_Q,\theta}(s,a)=\sqrt{m_Q}\tanh\!\left(\varphi_Q(s,a)^\top\theta/\sqrt{m_Q}\right).
 \label{eq:main-trained-critic}
\end{equation}
The scale $m_Q$ varies at fixed dimension $d_Q$. Section~\ref{sec:main-method} trains the critic; preferences use direct tuple estimates. Appendix~\ref{crex:example} verifies Assumptions A1, A2, G, and C1--C2 jointly for a continuous-state instance, implemented with a two-hidden-layer actor and five-feature critic in Appendix~\ref{app:continuous-validation}.

\paragraph{Response-chain correction.}
Hereafter suppress $\mathbf m$ and write $g=g_\tau$; subscripts $h_x,h_\alpha$ denote partial gradients of a differentiable function $h(x,\alpha)$. Let $D_x\alpha_0^*(x)\in\R^{r\times d_x}$ be the response Jacobian. The chain rule gives
\begin{equation}
 \nabla\Phi_\tau(x)=\nabla_x f(x,\alpha_0^*(x))
 +D_x\alpha_0^*(x)^\top\nabla_\alpha f(x,\alpha_0^*(x)).
 \label{eq:main-chain-rule}
\end{equation}
The second term accounts for policy adaptation. Section~\ref{sec:main-method} estimates it using first-order evaluations.
\FloatBarrier


==> sections/04_proposed_approach_updated.tex <==
\section{Proposed Approach}
\label{sec:main-method}

\paragraph{Response correction through paired actors.}
Following first-order penalty constructions \citep{kwon2024penalty}, let $\alpha_c^*(x)$ solve $g_\alpha+cf_\alpha=0$ locally in $\Bgeom$ for $0<c\le\min\{c_0,1\}$ and sufficiently small fixed $c_0$ (Section~\ref{sec:main-result}). Define
\begin{equation}
 S_c^*(x):=\frac{\alpha_c^*(x)-\alpha_0^*(x)}{c}.
 \label{eq:main-response-expansion}
\end{equation}
Persistent coordinates $U,S\in\R^r$ track $\alpha_0^*(x),S_c^*(x)$, with second actor $U+cS$. For $p=(x,U,S)$, set $a(p)=g_\alpha(x,U)$ and
\begin{align}
 R_c(p)&=\frac{g_\alpha(x,U+cS)-g_\alpha(x,U)}{c}+f_\alpha(x,U+cS),
 \label{eq:main-R}\\
 V_c(p)&=\frac{g_x(x,U+cS)-g_x(x,U)}{c}+f_x(x,U+cS).
 \label{eq:main-V}
\end{align}
At $U=\alpha_0^*(x)$ and $S=S_c^*(x)$, $R_c(p)=0$ and $V_c(p)=\nabla\Phi_\tau(x)+O(c)$ under Section~\ref{sec:main-result}'s conditions (Appendix~\ref{app:main-step-actor}). Gradient differences recover policy adaptation without evaluating Hessian inverses.

\paragraph{Paired critic and update geometry.}
Persistent critic coordinates $z=(u,v)\in\R^{2d_Q}$ specify $Q_{m_Q,u},Q_{m_Q,u+cv}$ for actors $U,U+cS$. Set $\eta_y=r_Q\beta$ and $\eta_x=q\eta_y$, with critic step $\beta>0$ and fixed positive ratios $r_Q,q$. Fix the chart, draw $n$ independent reset states by \eqref{klfin:eq:metric-size}, and certify their action-summed initialization covariance by \eqref{klfin:eq:accept}. On rejection return $x_0$; otherwise reuse $\widehat\rho_n$ for both actors, with uniform tube Fisher bounds (\cref{klfin:prop:Fisher}) and unchanged population objectives.

For a frozen base $b$ and direction $h$, define
\begin{equation}
 \ell_{b,h}(\alpha)=\frac1n\sum_{i=1}^n
 \KL\bigl(\pi_b(\cdot\mid s_i)\|\pi_\alpha(\cdot\mid s_i)\bigr)
 +\eta_y h^\top(\alpha-b).
 \label{eq:main-finite-KL}
\end{equation}
Let $\widetilde{\mathsf M}(b,h)$ run projected gradient descent on $\overline B(b,r_{\rm prox})$ from $b$ until $\|\nabla\ell_{b,h}\|\le m_{K,L}c\eta_y^2$. Certified curvature $m_{K,L}>0$ guarantees endpoint error $\le c\eta_y^2$ within $J_{\max}$ updates (\cref{klfin:prop:solver}). Appendix~\ref{app:support-prox} specifies the radius, step size, and finite action-sum gradient. Numerical iterations use no new environment draws. Use weighted critic projection $\Pi_{\mathcal K_Q}^{W}$ from \eqref{eq:algorithm-critic-update}. The test $\mathsf{Safe}(U,S)$ from \eqref{eq:safe} reserves the next actor-update buffer; failure returns $x_0$ with analytically controlled probability.

\paragraph{Sampling routines and timing.}
Algorithm~\ref{alg:deep} specifies routines and batches (Appendix~\ref{app:support-sampling}); rollout cap $H$ differs from preference length $K$. $\mathsf{LowerPair}$ uses paired critics and preference tuples to estimate $(a,R_c)$; set $\widehat C=\widehat a+c\widehat R$ exactly. $\mathsf{OuterPair}$ estimates $V_c$ using reward derivatives and separate preference tuples, without a value critic under fixed dynamics. $\mathsf{TDPair}$ reuses each base-policy transition for both endpoint residuals. All routines use frozen old parameters and conditionally independent blocks given pre-draw history, including the initial metric sample. Evaluation blocks use separate preference tuples and labels at the old perturbed actor; the new critic enters next iteration. Appendix~\ref{app:main-results} accounts for critic/truncation bias and all training/evaluation samples.

\begin{algorithm}[!t]
\caption{Single-loop bilevel RL with a persistent paired critic}
\label{alg:main-trained}
\small
\begin{algorithmic}[1]
\REQUIRE Initial $x_0\in\R^{d_x}$; $T,c,\tau,m_Q,H,\delta_{\rm met}$; batch sizes; step sizes
 $\beta,\eta_y=r_Q\beta,\eta_x=q\eta_y$; the specified geometry and radii.
\STATE Fix the chart; draw $n$ independent reset states to form $\widehat\rho_n$ and certify it using \eqref{klfin:eq:metric-size} and \eqref{klfin:eq:accept}.
\STATE Set $U_0=S_0=0$ and deterministic $z_0\in\mathcal K_Q$; \textbf{return} $x_0$ if the metric certificate or $\mathsf{Safe}(U_0,S_0)$ fails.
\FOR{$t=0,\ldots,T-1$}
 \STATE Freeze $p_t=(x_t,U_t,S_t)$ and $z_t$; retain $\dbar_t=\widehat\rho_n$.
 \STATE $(\widehat a_t,\widehat R_t)\gets\mathsf{LowerPair}(p_t,z_t;H)$;
 $\widehat C_t\gets\widehat a_t+c\widehat R_t$ exactly.
 \STATE $U_{t+1}\gets\widetilde{\mathsf M}(U_t,\widehat a_t)$;
 $\alpha^c_{t+1}\gets\widetilde{\mathsf M}(U_t+cS_t,\widehat C_t)$.
 \STATE $S_{t+1}\gets(\alpha^c_{t+1}-U_{t+1})/c$.
 \STATE $\widehat V_t\gets\mathsf{OuterPair}(p_t;H)$;
 $x_{t+1}\gets x_t-\eta_x\widehat V_t$.
 \STATE $\widehat F_t\gets\mathsf{TDPair}(p_t,z_t;H)$;
 $z_{t+1}\gets\Pi_{\mathcal K_Q}^{W}(z_t-\beta\widehat F_t)$.
 \STATE \textbf{return} $x_0$ if $\mathsf{Safe}(U_{t+1},S_{t+1})$ fails.
\ENDFOR
\STATE Draw an independent uniform index $J\in\{0,\ldots,T-1\}$; \textbf{return} $x_J$.
\end{algorithmic}
\end{algorithm}

\paragraph{Why shared samples matter.}
Let $\widehat d_0$ and $\widehat d_c$ denote sampled gradient
contributions at the actor endpoints $U$ and $U+cS$, respectively.
Define their centered sampling errors by
$\zeta_i=\widehat d_i-\E_t[\widehat d_i]$, $i\in\{0,c\}$,
where $\E_t$ conditions on the history before drawing the samples.
If the endpoint estimates use conditionally independent samples, then
$\frac{\E_t\|\zeta_c-\zeta_0\|^2}{c^2} =\frac{\E_t\|\zeta_c\|^2+\E_t\|\zeta_0\|^2}{c^2}$ with $\E_t$ conditioning on pre-draw history. Each evaluation rollout instead selects either endpoint policy with probability $1/2$, resets from $\rho$, and weights its shared trajectory by \eqref{eq:trained-prefix-weights}; paired TD shares base-policy transitions. Coupling controls normalized differences as $c$ shrinks (Appendices~\ref{app:support-sampling} and~\ref{app:main-step-tracking}). Direct preference terms are not divided by $c$.


==> sections/05_theoretical_analysis_updated.tex <==
\section{Theoretical Analysis}
\label{sec:main-result}
Fix $A>0$, $\overline B_A=\{\alpha\in\R^r:\|\alpha\|_2\le A\}$, and $0<R_{\rm geom}\le A/2$. Derivatives use multilinear operator norms, with order zero denoting the function. Bounds are uniform in admissible actor widths; after fixing the construction, global constants are independent of $x,c,m_Q$ and accuracy unless stated otherwise.

\begin{assumption}[A1: primitive local regularity]
\label{ass:regularity}\label{ass:main-primitive}
For every compact $Q\Subset\cO_x$ and $\alpha\in\overline B_A$, require:
\begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=2pt]
\item \textbf{Reward:} $r_x(s,a)$ is $C^4$ in $x$, with $\sup_{x\in Q,s,a}\|D_x^k r_x(s,a)\|\le C_{r,k}(Q)$ for $0\le k\le4$.
\item \textbf{Upper sample loss:} $L(x;\boldsymbol\xi,Y)$ is $C^4$ in $x$, with $\sup_{x\in Q,\boldsymbol\xi,Y}\|D_x^kL\|\le C_{L,k}(Q)$ for $0\le k\le4$.
\item \textbf{Actor score:} the normalized tied construction satisfies $\sup_{\mathbf m,\alpha\in\overline B_A,s,a}\|D_\alpha^kF_{\mathbf m,\alpha}\|\le C_{F,k}(A)$ for $1\le k\le4$.
\end{enumerate}
All envelopes are finite and uniform in sample arguments and admissible widths; state or action differentiability is unnecessary.
\end{assumption}
\noindent\emph{Context.} Related primitive and objective regularity appears in \citet[Assumption~2]{marbach2001} and \citet[Assumptions~2 and~7(2)]{kwon2024penalty}. Our fourth-order bounds control common-KL remainders; the architecture, beyond activation smoothness, verifies item~(iii).

\begin{assumption}[A2: initialization identifiability]
\label{ass:gap}\label{ass:main-population}
In the retained $r$-dimensional chart, let $Z_{\mathbf m,0}=D_\alpha F_{\mathbf m,0}$. For a width-independent $\lambda_{\rm eff,L}>0$, require
\begin{equation}
 \cG_{\mathbf m,0}:=\E_{s\sim\rho}
 \Cov_{a\sim\piRef(\cdot\mid s)}(Z_{\mathbf m,0}(s,a))
 \succeq\lambda_{\rm eff,L}I_r.
 \label{eq:main-population-gap}
\end{equation}
\end{assumption}


\noindent\emph{Context, verification, and derived geometry.}
Related Fisher nondegeneracy conditions appear in
\citet[Assumption~2.1]{liu2020} and
\citet[Assumption~3]{fatkhullin2023}, which impose positive Fisher bounds
throughout the actor parameter domain. A2 concerns the reset-distribution
covariance in the retained actor coordinates only at initialization.
It remains a primitive assumption in the general theorem. For a chart
fixed independently of the certification data, it admits a
high-probability finite-sample certificate
(\cref{red:prop:pilot-certification}); Appendix~\ref{crex:example}
verifies it analytically for an explicit neural construction.

The derivative bounds proved for the specified actor, together with the
global reward and loss bounds in G below, allow us to propagate this
initialization condition to a neighborhood. With sufficiently strong
fixed reference-KL regularization,
\cref{glob:geometry} derives
\begin{equation}
 \nabla_\alpha^2\!\left[
 g_{\tau,\mathbf m}(x,\alpha)+c f_{\mathbf m}(x,\alpha)
 \right]\succeq\mu_\tau I_r,
 \label{eq:main-derived-actor-curvature}
\end{equation}
for some $\mu_\tau>0$, uniformly in $x$, $\alpha\in\Bgeom$, and
$0\le c\le c_0$, yielding unique smooth local base and perturbed
responses. Under the additional critic conditions and the theorem's
schedule, the coupled containment analysis proves that the actor
iterates remain in this region with high probability
(\cref{critic:containment}). Thus local curvature, response regularity,
and containment are derived conclusions. The analysis uses the
initialization condition to justify the geometry needed along learning;
uniform lower-level PL is not assumed in the main theorem.


\begin{assumption}[G: global upper regularity for preference losses]
\label{ass:global-upper}
Use Section~\ref{sec:main-setup}'s fixed-dynamics, finite-action reset setting and objective~\eqref{eq:main-upper} on $\cO_x=\R^{d_x}$, with fixed tuple size $I$ and trajectory length $K$. Tuples and labels are freshly sampleable. The conditional feedback law is independent of $(x,\alpha)$ given the trajectories, and $L$ has no additional explicit actor dependence. For finite constants, uniformly in $x$ and sample arguments and for each realizable label we have,
\begin{equation}
 \begin{array}{lll}
 |r_x|\le B_r,&\|\nabla_xr_x\|\le G_r,&\|\nabla_x^2r_x\|_{\op}\le L_r,\\
 |L|\le B_L,&\|\nabla_xL\|\le G_L,&\|\nabla_x^2L\|_{\op}\le L_L.
 \end{array}
 \label{eq:main-global-envelopes}
\end{equation}


% Retain A1's local $C^4$ regularity; global bounds on pure third or fourth $x$ derivatives are unnecessary.
\end{assumption}
\noindent\emph{Context.} \citet[Assumptions~7.2--7.3]{yang2025bilevel} impose related global reward and finite-trajectory-loss envelopes. For Bradley--Terry, the reward bounds imply the loss envelopes (\cref{glob:BT}).

In C1--C2, the neighborhoods constructed in \cref{critic:containment} cover base and perturbed actors and prospective update segments for certificate~\eqref{eq:safe}.

\begin{assumption}[C1: fixed bounded critic features and excitation]
\label{ass:critic-features}
The map $\varphi_Q:\cS\times\cA\to\R^{d_Q}$ and dimension $d_Q$ are fixed independently of $x$, actors, $m_Q$, and accuracy, with $\sup_{s,a}\|\varphi_Q(s,a)\|\le F_Q<\infty$. Write $K_\alpha$ for the policy transition operator and $\nu_U$ for the normalized discounted reset occupancy in~\eqref{eq:critic-occupancy}. Every base actor $U$ in the stated neighborhood satisfies $\E_{\nu_U}[\varphi_Q\varphi_Q^\top]\succeq\lambda_QI_{d_Q}$ for a uniform $\lambda_Q>0$.
\end{assumption}
\noindent\emph{Context.} Related feature conditions appear in linear TD \citep[Section~2]{bhandari2018td} and neural TD \citep[Assumption~3.1]{ke2024td}; C1 requires a full Gram gap under discounted reset occupancy.

\begin{assumption}[C2: realizability of the regularized lower value]
\label{ass:critic-realizability}
Choose sufficiently large finite $\tau$ for actor geometry and initialization as in \cref{glob:geometry,critic:containment}, then keep it fixed before selecting critic constants. At this value, for every $x\in\R^{d_x}$ and actor $\alpha$ in the stated neighborhood, require
\begin{equation}
 \begin{gathered}
 q_{x,\alpha}(s,a)=-r_x(s,a)
       +\tau\log\frac{\pi_\alpha(a\mid s)}{\piRef(a\mid s)},\\
 Q^{\mathrm{true}}_{x,\alpha}=(\mathrm{Id}-\gamma K_\alpha)^{-1}q_{x,\alpha}
       \in\operatorname{span}\varphi_Q,
 \end{gathered}
 \label{eq:regularized-value}
\end{equation}
where $\mathrm{Id}$ is the identity operator and $\operatorname{span}\varphi_Q=\{\varphi_Q^\top b:b\in\R^{d_Q}\}$.
\end{assumption}
\noindent\emph{Context.} Related value-representation conditions appear in \citet[Assumption~A and Proposition~2.3]{jin2020linear}; neural TD can retain projection error \citep[Theorem~3.7]{ke2024td}. C2 concerns the entire \emph{regularized} value family at fixed $\tau$, including the policy-dependent KL cost.


\paragraph{Paired accuracy of the nonlinear critic.}
Under the stated assumptions, the critic~\eqref{eq:main-trained-critic}
has stable paired population TD targets
(\cref{critic:TD-stability,critic:pair-global}). For $p=(x,U,S)$, let
$(u^*,v^*)=Z(p)$ denote the paired target defined in~\eqref{critic:Z},
and define its value errors by
\[
\begin{aligned}
 e_0^*(p)&=Q_{m_Q,u^*}-Q^{\mathrm{true}}_{x,U},\\
 e_c^*(p)&=Q_{m_Q,u^*+cv^*}-Q^{\mathrm{true}}_{x,U+cS}.
\end{aligned}
\]
Appendix~\ref{app:main-step-td} derives the paired approximation floor
\begin{equation}
 \mathcal A_Q:=\sup_p\left\{
 \|e_0^*(p)\|_\infty^2+
 \left\|\frac{e_c^*(p)-e_0^*(p)}{c}\right\|_\infty^2
 \right\}\le C m_Q^{-2},
 \label{eq:main-paired-critic-floor}
\end{equation}
where the supremum ranges over the prescribed actor neighborhoods and all
$x$, and $C$ is independent of $c$ and $m_Q$ in their admissible ranges.
The proof controls both the approximation error and its variation with
the actor, so endpoint-error differences are $O(c/m_Q)$ before division
by $c$ (\cref{critic:paired-floor}). Separate $O(m_Q^{-1})$ endpoint
estimates would yield only an $O(m_Q^{-2}c^{-2})$ bound for the squared
normalized difference. With $c^2=\Theta(\varepsilon)$ and
$m_Q=\Theta(\varepsilon^{-1/2})$, that bound is $O(1)$, whereas
\eqref{eq:main-paired-critic-floor} gives $O(\varepsilon)$. This floor concerns population TD targets. Algorithm~\ref{alg:main-trained}
learns them through persistent projected updates from any deterministic
$z_0\in\mathcal K_Q$. The coupled tracking analysis controls the additional
error from sampling, finite updates, and changing rewards and actors,
and includes critic training in the final interaction bound
(Appendices~\ref{app:main-step-tracking} and~\ref{app:main-step-stationarity}).
The scale $m_Q$ controls nonlinearity at fixed feature dimension.


% \begin{theorem}[Single-loop stationarity with a trained paired critic]
% \label{thm:main}\label{thm:main-headline}
% Use the specified actor and critic~\eqref{eq:main-trained-critic}, with fixed actor depth, retained actor dimension, and critic feature dimension. Assume A1, A2, G, and C1--C2 at the selected fixed $\tau$ and actor neighborhoods. Initialize $U_0=S_0=0$ and any deterministic $z_0\in\mathcal K_Q$. Run Algorithm~\ref{alg:main-trained}, including its sampling, projected TD, certified empirical metric, and residual-controlled KL solves, with metric rejection budget $\delta_{\rm met}=\eps/2$.

% There are fixed critic projection radii, actor buffers, positive ratios $r_Q,q$, and positive constants $k_\beta,k_c,k_T,m_{Q,0},C_m$ such that, for sufficiently small $\eps>0$, use
% \begin{equation}
%  \begin{gathered}
%  \beta=k_\beta\eps,\quad \eta_y=r_Q\beta,\quad
%  \eta_x=q\eta_y,\quad c^2=k_c\eps,\quad T=\lceil k_T\eps^{-2}\rceil,\\
%  H=\Theta\!\left((1-\gamma)^{-1}\log(1/\eps)\right),\qquad
%  m_Q\ge\max\{m_{Q,0},C_m\eps^{-1/2}\}.
%  \end{gathered}
%  \label{eq:main-schedule}
% \end{equation}
% Choose the horizon constant large enough that the squared TD and evaluation truncation biases sum to $o(\eps)$, with positive TD/evaluation batches bounded by a fixed polynomial in $H$ (including fixed batches; Appendix~\ref{app:support-sampling}) and fixed preference batches. Conditionally on metric acceptance, actor containment through $T$ holds with probability at least $1-\delta_a$, where $\delta_a=\eps/2$; total failure probability is at most $\eps$.

% Let $x_{\rm out}=x_J$ for independent $J\sim\mathrm{Unif}\{0,\ldots,T-1\}$ if neither the metric nor an actor certificate fails, and $x_{\rm out}=x_0$ otherwise. Let $N_{\rm seg},N_{\rm trans}$ count all sampled trajectory segments and environment transitions. For fixed $\gamma,I,K$,
% \begin{equation}
%  \E\|\nabla\Phi_{\tau,\mathbf m}(x_{\rm out})\|^2=O(\eps),
%  \qquad N_{\rm seg},N_{\rm trans}=\widetilde{\mathcal O}(\eps^{-2}).
%  \label{eq:main-headline-bound}
% \end{equation}
% The counts include TD, evaluation, preference, and the $n=O(\log(1/\eps))$ initial metric states; any separate pilot is charged once. Labels cost $O(\eps^{-2})$. With $\kappa_K=M_{K,L}/m_{K,L}$, the two local solves per iteration use at most
% \begin{equation}
%  N_{\mathrm{KL\text{-}grad}}\le2T(J_{\max}+1)
%  =O\!\left(\kappa_K\eps^{-2}\log(1/\eps)\right)
%  \label{eq:main-KL-work}
% \end{equation}
% finite-sum gradients, each on $n|\cA|$ stored state--action terms.
% The tilde suppresses logarithmic factors in $1/\eps$.
% \end{theorem}
% The response exists for every $x\in\R^{d_x}$. The criterion uses squared hypergradient norm; numerical KL work is separate from interactions.

\begin{theorem}[Single-loop stationarity with a trained paired critic]
\label{thm:main}\label{thm:main-headline}
Fix $\gamma,I,K$, the actor depth and retained dimension, and the
critic feature dimension. Assume A1, A2, G, and C1--C2 for the
specified actor and critic~\eqref{eq:main-trained-critic}, at the
selected fixed $\tau$ and actor neighborhoods.
Initialize $U_0=S_0=0$ and any deterministic
$z_0\in\mathcal K_Q$, where $\mathcal K_Q$ is the critic projection
set defined in Appendix~\ref{app:main-step-td}.

There exist fixed projection radii, actor buffers, positive step
ratios $r_Q,q$, and positive constants independent of $\eps$ such
that, for all sufficiently small $\eps>0$, the following schedule
is admissible:
\begin{equation}
 \begin{gathered}
 \beta=k_\beta\eps,\qquad
 \eta_y=r_Q\beta,\qquad
 \eta_x=q\eta_y,\qquad
 c^2=k_c\eps,\qquad
 T=\lceil k_T\eps^{-2}\rceil,\\
 H=\Theta\!\left((1-\gamma)^{-1}\log(1/\eps)\right),
 \qquad
 m_Q\ge\max\{m_{Q,0},C_m\eps^{-1/2}\}.
 \end{gathered}
 \label{eq:main-schedule}
\end{equation}
Choose the fixed constants as in
Appendix~\ref{app:main-step-containment}, with a sufficiently large
horizon constant so that squared truncation biases sum to $o(\eps)$.
Use positive TD and evaluation batches at most polynomial in $H$
and fixed preference batches, following
Appendix~\ref{app:support-sampling}.

Run Algorithm~\ref{alg:main-trained} with this schedule and
$\delta_{\rm met}=\eps/2$, including its certified metric and
finite KL solves. The total certificate-failure probability is
at most $\eps$. Its output $x_{\rm out}$, chosen uniformly among
the training iterates on success and equal to $x_0$ otherwise,
satisfies
\begin{equation}
 \E\|\nabla\Phi_{\tau,\mathbf m}(x_{\rm out})\|^2=O(\eps),
 \qquad
 N_{\rm seg},N_{\rm trans}
 =\widetilde{\mathcal O}(\eps^{-2}),
 \label{eq:main-headline-bound}
\end{equation}
where $N_{\rm seg},N_{\rm trans}$ count all sampled trajectory
segments and environment transitions, including critic training,
evaluation, preference sampling, and initialization data.
% The label count is $O(\eps^{-2})$, and the tilde suppresses
% logarithmic factors in $1/\eps$.
\end{theorem}

Appendix~\ref{app:support-prox} specifies the metric certificate
and finite KL solvers.
Appendix~\ref{app:main-step-stationarity} proves the theorem and
provides complete interaction and numerical-work accounting.


\paragraph{Interpretation of the guarantee.}
\Cref{thm:main-headline} accounts for learning the specified nonlinear
critic jointly with the two actor responses and the upper variable.
It permits any deterministic critic initialization in $\mathcal K_Q$;
the analysis controls the ensuing tracking error as rewards and policies
change. Shared trajectories control normalized sampling noise, while
the paired critic analysis controls approximation-error differences
after division by the shrinking response perturbation. Together with
derived actor geometry and proved containment, these estimates establish
the $\widetilde{\mathcal O}(\varepsilon^{-2})$ interaction bound with
persistent critic training under the stated conditions. The count
includes critic, evaluation, preference, and initialization samples.


The conclusion is stationarity of the upper objective induced by a
selected local policy response at fixed reference-KL regularization.
Under an additional PL condition on a prescribed actor domain,
Appendix~\ref{app:gpl-global-response} shows that this response is a
global minimizer of the regularized lower objective.
% on that domain.
% The upper-level guarantee remains stationarity, with the same
% interaction bound.
% the upper-level conclusion remains stationarity.
% Appendix~\ref{app:support-prox} specifies the metric certificate and
% finite KL solvers, and Appendix~\ref{app:main-step-stationarity}
% provides the proof and complete interaction and numerical-work accounting.



% \subsection{Proof outline}
% \label{subsec:main-proof-outline}
% Write $\Phi=\Phi_{\tau,\mathbf m}$. We derive uniform bounds
% $\|\nabla\Phi\|\le G_\Phi$ and $\Phi\ge\underline\Phi$, where
% $\underline\Phi=0$ for Bradley--Terry and $-B_L$ otherwise
% (\cref{critic:actor-field-bounds}). Appendix~\ref{app:main-results}
% follows these six steps.

% \paragraph{1. Actor geometry and response correction.}
% (Appendix~\ref{app:main-step-actor}.) A2, the occupancy's reset component,
% and network derivative bounds give local reference-KL curvature.
% Sufficient fixed $\tau$ yields unique interior base and perturbed responses
% uniformly in $x$ (\cref{glob:geometry}). First-order evaluations give
% $V_c(x,\alpha_0^*(x),S_c^*(x))=\nabla\Phi(x)+O(c)$
% (\cref{glob:secant}). This step establishes that the ideal first-order update approximates the
% true upper gradient, providing the reference against which subsequent
% policy-tracking and estimation errors are controlled.

% \paragraph{2. Stable paired TD targets and derived accuracy.}
% (Appendix~\ref{app:main-step-td}.) The reset identity and Jensen's inequality give
% \begin{equation}
%  \E_{\nu_U}[h(h-\gamma K_Uh)]
%  \ge(1-\sqrt\gamma)\|h\|_{L^2(\nu_U)}^2
%  \label{eq:outline-coercivity}
% \end{equation}
% for square-integrable $h$. With $h=\varphi_Q^\top b$, C1 transfers this
% coercivity to the linear TD matrix. The $O(c)$ actor perturbation and
% $O(m_Q^{-1})$ critic nonlinearity preserve stability, yielding an interior
% paired-TD root $Z(p)$ with two bounded derivatives
% (\cref{critic:TD-stability,critic:pair-global}). C2 gives
% $\mathcal A_Q=O(m_Q^{-2})$ for squared base error and normalized
% endpoint-error difference (\cref{critic:paired-floor}).
% This step provides stable, smoothly varying critic targets and controls
% their approximation errors even after division by $c$, establishing the
% foundation for bounding the critic's contribution to the upper-gradient error.

% \paragraph{3. Shared samples, finite KL solves, and persistent tracking.}
% (Appendix~\ref{app:main-step-tracking}.) Shared endpoint differences are
% $O(c)$ before division, keeping normalized moments bounded. A segment-integral
% argument needs global upper derivatives only through order two
% (\cref{critic:anisotropic}). Evaluation uses the old critic and
% $\widehat C=\widehat a+c\widehat R$; independent TD tracks $Z(p)$
% (\cref{critic:oracle,critic:moving,critic:recursions}). Conditional
% independence cancels centered target-movement cross terms, so only mean
% drift incurs a $1/\beta$ penalty. The empirical metric certificate preserves
% local KL curvature. Residual-controlled solves have endpoint error
% $c\eta_y^2$ and normalized error $O(\eta_y^2)$, absorbed into tracking
% remainders without new samples (\cref{klfin:prop:solver,klfin:prop:transfer}).This step controls the errors from sampling, finite actor solves, and
% critic tracking, connecting the ideal response correction to the
% implemented updates.

% \paragraph{4. A contracting potential for containment.}
% (Appendix~\ref{app:main-step-contraction}.) Combine critic error
% $\mathcal C_t=\|z_t-Z(p_t)\|_W^2$ and the actor tracking potential
% $\mathcal T_t$ from~\eqref{critic:actor-potential}:
% \begin{equation}
%  \mathcal D_t=\mathcal T_t+\lambda r_Q\mathcal C_t,
%  \qquad \lambda>0.
%  \label{eq:outline-D}
% \end{equation}
% For small fixed step ratios, \cref{critic:fast} gives, through a prospective exit,
% \begin{equation}
%  \E_t\mathcal D_{t+1}\le(1-\rho_D\eta_y)\mathcal D_t
%  +C_D\eta_y(qG_\Phi^2+\omega+\beta),\quad
%  \omega=c^2+\mathcal A_Q+b_{\rm ev}^2+b_{\rm TD}^2.
%  \label{eq:outline-drift}
% \end{equation}
% Here $\E_t$ conditions on pre-draw history and the accepted metric;
% $b_{\rm ev},b_{\rm TD}$ bound truncation biases. Small $q$ controls target
% movement for containment; $qG_\Phi^2$ does not enter the stationarity floor.
% This step controls actor and critic errors jointly despite their mutual
% dependence, supplying the contraction bound needed to establish
% containment in the certified region.This step ensures that the iterates remain in the certified region
% throughout training with high probability, making the preceding local
% guarantees valid for the subsequent convergence analysis.

% \paragraph{5. Constructively excluding a first exit.}
% (Appendix~\ref{app:main-step-containment}.) Choose geometry and fixed $\tau$,
% critic constants and weights, then $r_Q$ for initial critic error and $q$
% for target movement. A stopped martingale bound controls $\mathcal D_t$
% through a prospective exit. Under~\eqref{eq:main-schedule}, fluctuations
% vanish as $\sqrt{\eta_y\log(T/\eps)}\operatorname{poly}(H)$ and fit
% inside the actor buffers, excluding exit with conditional probability
% $1-\eps/2$ (\cref{critic:D-max,critic:containment}). Prospective bounds
% precede containment; projection contains the critic and G removes upper exits.

% \paragraph{6. Stationarity and complete data accounting.}
% (Appendix~\ref{app:main-step-stationarity}.) For fixed positive weights,
% \cref{critic:master} combines upper descent and tracking into
% \begin{equation}
%  \begin{aligned}
%  \Psi_t&=\Phi(x_t)-\underline\Phi+a_\Psi q\mathcal T_t+b_\Psi qr_Q\mathcal C_t,\\
%  \E_t\Delta\Psi_t&\le-a_*\eta_x(\|\nabla\Phi(x_t)\|^2+\mathcal T_t+\mathcal C_t)
%        +C_*\eta_x(\omega+\beta+\eta_y+\eta_x).
%  \end{aligned}
%  \label{eq:outline-Psi}
% \end{equation}
% Weights and step ratios absorb the cross terms. Telescoping with the
% pre-draw no-exit indicator, random output, and the failure bound yields
% \begin{equation}
%  \E\|\nabla\Phi(x_{\rm out})\|^2
%  \le C\left[\frac{\Psi_0}{\eta_xT}+\omega+\beta+\eta_y+\eta_x\right]
%        +\eps G_\Phi^2.
%  \label{eq:outline-final-rate}
% \end{equation}
% Nonnegativity avoids conditioning on future containment; $\Psi_0$ includes
% initial critic error. Schedule~\eqref{eq:main-schedule} makes every term
% $O(\eps)$. Counting metric, TD, evaluation, and preference data gives the
% interaction bound.

\subsection{Proof outline}
\label{subsec:main-proof-outline}
Write $\Phi=\Phi_{\tau,\mathbf m}$. The derived bounds
$\|\nabla\Phi\|\le G_\Phi$ and $\Phi\ge\underline\Phi$ hold globally
in $x$, with $\underline\Phi=0$ for Bradley--Terry and $-B_L$ otherwise
(\cref{critic:actor-field-bounds}). Appendix~\ref{app:main-results}
follows the six steps below.
% Conditional expectations $\E_t$ use the
% pre-draw history, including the accepted initial metric sample. Local
% one-step bounds are established before invoking the containment result.

\paragraph{1. Derived actor geometry and first-order response correction.}
(Appendix~\ref{app:main-step-actor}.) A2, the reset component of occupancy,
and the architectural derivative bounds yield local reference-KL
curvature. Sufficiently strong fixed $\tau$ dominates the reward and
perturbation curvature, giving unique smooth interior base and perturbed
responses uniformly in $x$ (\cref{glob:geometry}). Their normalized
difference yields
$V_c(x,\alpha_0^*(x),S_c^*(x))=\nabla\Phi(x)+O(c)$
(\cref{glob:secant}). This identifies the first-order population
direction to be tracked, with squared response-approximation error
$O(c^2)$ and without assuming uniform lower-level PL.

\paragraph{2. Stable paired TD targets and normalized approximation errors.}
(Appendix~\ref{app:main-step-td}.) The reset identity and Jensen's
inequality give, for square-integrable $h$,
\begin{equation}
 \E_{\nu_U}[h(h-\gamma K_Uh)]
 \ge(1-\sqrt\gamma)\|h\|_{L^2(\nu_U)}^2.
 \label{eq:outline-coercivity}
\end{equation}
C1 transfers this coercivity to the linear-feature TD system.
Controlling the $O(c)$ actor perturbation and the $O(m_Q^{-1})$
nonlinear field and derivative perturbations preserves stability,
yielding an interior paired target $Z(p)$ with bounded first and
second derivatives (\cref{critic:TD-stability,critic:pair-global}).
Under C2, comparing both the TD roots and their actor derivatives
with the linear realizable values gives endpoint-error differences
of order $c/m_Q$. Thus the squared base and normalized-difference
approximation floor is $\mathcal A_Q=O(m_Q^{-2})$
(\cref{critic:paired-floor}). This controls approximation at the
population targets.
% the next step treats finite training.

\paragraph{3. Shared samples, finite solves, and moving-target tracking.}
(Appendix~\ref{app:main-step-tracking}.) Shared-trajectory weighting
keeps normalized sampling moments bounded uniformly in $c$.
Evaluation uses the old critic and the compatible fields
$\widehat C=\widehat a+c\widehat R$; conditionally independent TD
updates track $Z(p)$ (\cref{critic:oracle,critic:recursions}).
Centering the random target movement cancels its linear cross term,
so only conditional mean drift incurs a $1/\beta$ penalty
(\cref{critic:moving}). The empirical metric certificate and finite
KL solvers give endpoint parameter error at most $c\eta_y^2$, hence
normalized solver error $O(\eta_y^2)$, using stored states
(\cref{klfin:prop:solver,klfin:prop:transfer}). 
% These estimates yield
% coupled recursions for actor tracking, critic tracking, and upper descent.

\paragraph{4. Joint tracking contraction.}
(Appendix~\ref{app:main-step-contraction}.) Let
$\mathcal C_t=\|z_t-Z(p_t)\|_W^2$ and let $\mathcal T_t$ be the actor
potential in~\eqref{critic:actor-potential}. For a fixed positive weight, $\mathcal D_t=\mathcal T_t+\lambda r_Q\mathcal C_t.$
Choosing sufficiently small fixed step ratios absorbs the mutual
actor--critic error terms and gives (\cref{critic:fast})
\begin{equation}
 \E_t\mathcal D_{t+1}\le(1-\rho_D\eta_y)\mathcal D_t
 +C_D\eta_y(qG_\Phi^2+\omega+\beta),\qquad
 \omega=c^2+\mathcal A_Q+b_{\rm ev}^2+b_{\rm TD}^2,
 \label{eq:outline-drift}
\end{equation}
where $b_{\rm ev},b_{\rm TD}$ bound truncation biases. This drift
inequality holds before exit and through the prospective next step in
the larger analytic neighborhood. The $qG_\Phi^2$ term bounds target
movement for containment; Step~6 retains the gradient term explicitly
to avoid introducing this constant into the stationarity floor.

\paragraph{5. Proving containment of the coupled iterates.}
(Appendix~\ref{app:main-step-containment}.) Choose actor geometry and
fixed $\tau$, then critic radii and potential weights, followed by
$r_Q$ to accommodate the permitted initial critic error and $q$ to
control target drift. Buffered prospective-step estimates justify the
local recursions before containment is known. A stopped martingale
bound then controls $\mathcal D_t$: under~\eqref{eq:main-schedule},
fluctuations of order
$\sqrt{\eta_y\log(T/\eps)}\operatorname{poly}(H)$ fit inside the
actor buffers. This excludes a first actor exit with conditional
probability at least $1-\eps/2$ for every accepted metric realization
(\cref{critic:D-max,critic:containment}). Projection contains the
critic, and G supplies global bounds in the upper variable.

\paragraph{6. Upper stationarity and complete interaction accounting.}
(Appendix~\ref{app:main-step-stationarity}.) Add upper-objective descent
to the tracking recursions with fixed positive weights. With
$\Delta\Psi_t=\Psi_{t+1}-\Psi_t$, \cref{critic:master} gives
\begin{equation}
 \begin{aligned}
 \Psi_t&=\Phi(x_t)-\underline\Phi
       +a_\Psi q\mathcal T_t+b_\Psi qr_Q\mathcal C_t,\\
 \E_t\Delta\Psi_t
 &\le-a_*\eta_x\bigl(\|\nabla\Phi(x_t)\|^2
                       +\mathcal T_t+\mathcal C_t\bigr)
       +C_*\eta_x(\omega+\beta+\eta_y+\eta_x).
 \end{aligned}
 \label{eq:outline-Psi}
\end{equation}
Telescoping with the predictable pre-exit indicator and using
nonnegativity of the terminal potential avoids conditioning on future
successful training. The independent uniform output on success and
the fallback $x_0$ on failure, with total failure probability at most
$\eps$, give
\begin{equation}
 \E\|\nabla\Phi(x_{\rm out})\|^2
 \le C\left[\frac{\Psi_0}{\eta_xT}
                  +\omega+\beta+\eta_y+\eta_x\right]
       +\eps G_\Phi^2.
 \label{eq:outline-final-rate}
\end{equation}
The initial potential includes the initial critic error, and
schedule~\eqref{eq:main-schedule} makes every term $O(\eps)$.
Counting all TD, evaluation, preference, metric, and optional pilot
samples yields $\widetilde{\mathcal O}(\eps^{-2})$ interactions.
% Finite KL iterations reuse stored metric states; their numerical
% work is accounted for separately.

==> sections/06_main_results_one_page_updated.tex <==
% \section{Empirical Results}
% \label{sec:empirical-results}
% \vspace{-0.4em}
% \subsection{Theory-aligned continuous-state validation}
% \label{sec:continuous-validation}
% \vspace{-0.25em}
% We sample Appendix~\ref{crex:example}'s continuous-state construction:
% $s\in[-1,1]$, two actions, a tied two-hidden-layer actor, and a five-feature
% nonlinear paired critic. Appendices~\ref{app:continuous-validation}
% and~\ref{app:implementation-differences} give protocols and certification qualifications.

% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{figures/empirical_headline_compact.pdf}
% \vspace{-0.6em}
% \caption{Continuous-state validation. (a) Secant bias at four points.
% (b) Paired-TD variance, matched cost (200 batches). (c) Squared TD-root error,
% $c=0.05$; $m_Q$ varies with five coordinates fixed. (d) Uniform-output
% stationarity, ten seeds, 95\% $t$ intervals, and an $N^{-1/2}$ reference.}
% \label{fig:continuous-headline}
% \end{figure}
% \vspace{-0.4em}
% \paragraph{Response and critic mechanisms.}
% Secant-bias slopes are $0.9996$--$0.9999$; representative paired-TD variance
% slopes are $0.051$ (shared) and $-2.005$ (independent).
% The 120 TD-root cells show approximately $m_Q^{-2}$ squared error.
% From displaced critic initialization, mean weighted tracking error falls
% from $416$ to $0.1904$ and squared paired value error from $23.77$ to
% $4.44\times10^{-4}$, supporting nonlinear critic learning.

% \paragraph{Interaction scaling and controls.}
% Across four budgets and two initializations, we plot uniform-output
% stationarity $\overline G_T=T^{-1}\sum_{t<T}|\Phi'(x_t)|^2$ against
% all training transitions plus initial metric states. An eightfold interaction increase
% reduces mean stationarity by about $2.86$ for both initializations
% (slopes $-0.505$). This finite-range consistency is transient-dominated:
% over $99.9\%$ of gradient mass occurs in the first half. Population controls
% isolate the correction; sampled final-stationarity superiority is unresolved,
% and fixed-budget average stationarity is slightly worse with correction.

% \subsection{End-to-end continuous-state benchmarks}
% \vspace{-0.25em}
% Table~\ref{tab:end-to-end-summary} uses five matched seeds, 100k main
% interactions, and 500 labels per preference method. Auxiliary transitions
% total 9,216 on Walker and 1,578--1,800 on Highway. Secant improves mean
% Walker return over the adapted value-only comparator; Highway means are similar.
% Known-reward SAC uses task rewards; details are in
% Appendices~\ref{app:end-to-end-details}--\ref{app:implementation-differences}.

% \begin{table}[h]
% \centering
% \setlength{\tabcolsep}{5pt}
% \caption{Final return: mean $\pm$ SD over five seeds; ten evaluation episodes per seed.}
% \label{tab:end-to-end-summary}
% \begin{tabular}{@{}lrrr@{}}
% \toprule
% Task & Secant & Gaur adaptation & Known-reward SAC\\
% \midrule
% Walker Walk & $334.43\pm84.67$ & $131.66\pm101.74$ & $794.36\pm39.48$\\
% Highway-fast & $35.01\pm0.29$ & $35.03\pm0.31$ & $34.96\pm0.25$\\
% \bottomrule
% \end{tabular}
% \end{table}

\section{Empirical Results}
\label{sec:empirical-results}

We examine two questions: whether the analyzed neural construction exhibits
the predicted dependence on environment interactions, and whether a
practical adaptation performs effectively in an end-to-end continuous
control task. Additional mechanism studies and implementation details
appear in the appendix.

\subsection{Interaction scaling for the analyzed construction}
\label{sec:continuous-validation}

We use the continuous-state construction in
Appendix~\ref{crex:example}, with a tied two-hidden-layer actor and a
five-feature nonlinear critic trained from sampled data.
The theoretical interaction bound
$\widetilde{\mathcal O}(\varepsilon^{-2})$ corresponds to
$\widetilde{\mathcal O}(N^{-1/2})$ decay of expected squared
upper-gradient norm. We therefore measure
\[
 \overline G_T
 =\frac{1}{T}\sum_{t=0}^{T-1}|\Phi'(x_t)|^2
\]
against the total interaction count $N$, including all training
transitions and initial metric states. This average evaluates the
theorem's uniform-output stationarity criterion.

Across four budgets and ten matched seeds, an eightfold increase in
interactions reduces mean stationarity by approximately $2.86$,
close to the $\sqrt{8}$ reduction suggested by the predicted scaling.
The fitted log--log slopes are approximately $-0.505$ for both zero
and displaced critic initialization. These results support finite-budget
consistency with the interaction bound, including when the critic starts
from inaccurate value estimates. The average is dominated by the early
training transient, which limits conclusions about asymptotic scaling
and the separate contributions of individual error terms.
Appendix~\ref{app:continuous-validation} provides the full protocol,
uncertainty estimates, and diagnostic results.

\subsection{End-to-end learning on Walker Walk}
\label{sec:walker-main}

We next evaluate a practical adaptation on Walker Walk, which has
continuous observations and actions. The implementation combines neural
reward learning with SAC and uses the response correction in the upper
update. Both preference-based methods use 100,000 main interactions,
500 preference labels, and 9,216 auxiliary response interactions.
Learning curves report returns against total training interactions.

Across five matched training seeds, our method achieves a final return
of $334.43\pm84.67$, compared with $131.66\pm101.74$ for the adapted
value-only comparator based on \citet{gaur2025sample}. Values are means
and sample standard deviations across seeds, with ten evaluation episodes
per seed. SAC trained directly on the known task reward achieves
$794.36\pm39.48$ and provides a reference with privileged reward access.

The higher mean return relative to the adapted comparator supports the
practical applicability of the response correction in this end-to-end
setting. The experiment uses broader architectures and update rules than
the analyzed construction; Appendix~\ref{app:implementation-differences}
documents these differences. Full learning curves, the six-seed
sensitivity analysis, and additional benchmark results are provided in
Appendix~\ref{app:end-to-end-details}.



==> tables/highway_fast_checkpoints.tex <==
\begin{table}[ht]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Highway-fast: evaluation return, mean $\pm$ sample SD across five training seeds.}
\label{tab:highway_fast-checkpoints}
\begin{tabular}{@{}lrrr@{}}
\toprule
Main steps & Secant & Gaur et al. & Known-reward SAC \\
\midrule
25k & $36.92\pm2.71$ & $35.21\pm0.33$ & $35.41\pm1.13$ \\
50k & $35.17\pm0.28$ & $35.25\pm0.72$ & $35.45\pm0.55$ \\
75k & $34.76\pm0.19$ & $34.92\pm0.62$ & $35.13\pm0.45$ \\
100k & $35.01\pm0.29$ & $35.03\pm0.31$ & $34.96\pm0.25$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/highway_fast_seeds.tex <==
\begin{table}[ht]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Highway-fast: final per-training-seed mean return over ten evaluation episodes.}
\label{tab:highway_fast-seeds}
\begin{tabular}{@{}lrrr@{}}
\toprule
Training seed & Secant & Gaur et al. & Known-reward SAC \\
\midrule
1 & 35.10 & 35.18 & 35.33 \\
3 & 34.72 & 35.09 & 35.03 \\
4 & 35.38 & 34.90 & 34.99 \\
5 & 34.70 & 34.58 & 34.74 \\
6 & 35.15 & 35.39 & 34.71 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/walker_walk_checkpoints.tex <==
\begin{table}[ht]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Walker Walk: evaluation return, mean $\pm$ sample SD across five training seeds.}
\label{tab:walker_walk-checkpoints}
\begin{tabular}{@{}lrrr@{}}
\toprule
Main steps & Secant & Gaur et al. & Known-reward SAC \\
\midrule
25k & $112.90\pm39.49$ & $34.30\pm18.84$ & $286.40\pm40.06$ \\
50k & $132.99\pm86.18$ & $73.41\pm40.85$ & $507.76\pm73.68$ \\
75k & $291.63\pm83.79$ & $125.45\pm92.75$ & $720.04\pm60.60$ \\
100k & $334.43\pm84.67$ & $131.66\pm101.74$ & $794.36\pm39.48$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/walker_walk_seeds.tex <==
\begin{table}[ht]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{Walker Walk: final per-training-seed mean return over ten evaluation episodes.}
\label{tab:walker_walk-seeds}
\begin{tabular}{@{}lrrr@{}}
\toprule
Training seed & Secant & Gaur et al. & Known-reward SAC \\
\midrule
1 & 336.10 & 123.28 & 746.43 \\
3 & 194.04 & 103.20 & 806.89 \\
4 & 421.90 & 77.25 & 761.95 \\
5 & 359.78 & 48.06 & 842.96 \\
6 & 360.34 & 306.50 & 813.60 \\
\bottomrule
\end{tabular}
\end{table}

